On Minimax Optimality of Sparse Bayes Predictive Density Estimates

We study predictive density estimation under Kullback-Leibler loss in $\ell_0$-sparse Gaussian sequence models. We propose proper Bayes predictive density estimates and establish asymptotic minimaxity in sparse models. A surprise is the existence of a phase transition in the future-to-past variance ratio $r$. For $r < r_0 = (\surd 5 - 1)/4$, the natural discrete prior ceases to be asymptotically optimal. Instead, for subcritical $r$, a `bi-grid' prior with a central region of reduced grid spacing recovers asymptotic minimaxity. This phenomenon seems to have no analog in the otherwise parallel theory of point estimation of a multivariate normal mean under quadratic loss. For spike-and-slab priors to have any prospect of minimaxity, we show that the sparse parameter space needs also to be magnitude constrained. Within a substantial range of magnitudes, spike-and-slab priors can attain asymptotic minimaxity.

==> document.tex <==
\subsection{Proofs of the Lemmas used in Section~\ref{sec-2-3}} 
\noindent \textbf{Proof of Lemma~\ref{lem-SS-1}.} We prove the lemma for positive parameter values. By symmetry, the proof easily extends over to the general case. As $\vw\le 1$, by definition \eqref{eq:SS-decomp-1a},
$\ex\{\log(1+N^s_{\theta}(Z))\}$ is bounded above by 
\begin{equation*}
\ex [\log(1+c(\eta)\,\exp{(\vw W^2/2)}\,\Phi(\vwmh(l-\theta)-Z))]~.
\end{equation*}
\noindent Now noting that $\vw W^2=\vw^{-1}\theta^2+Z^2+2\vw^{-1/2}\theta Z$ the above is bounded by 
\begin{equation*}
\ex\big[\log\big\{1+c(\eta)\exp(\vw^{-1}\theta^2/2)\Phi(\vwmh(l-\theta)-Z)\big\}\big]+2^{-1}\big[\ex(Z^2)+2\vwmh\,\theta\,\ex|Z|\big]~.
\end{equation*}
\noindent As $\ex(Z^2)=1$ and $\ex|Z|=2\phi(0)$, we concentrate on the first term in the above display. Consider
the event $A=\{Z:\vwmh(l-\theta)-Z\ge-1\}$. For  $ Z \in A^c$, note that 
\begin{align*}
\Phi(\vwmh(l-\theta)-Z)&\le\phi(\vwmh(l-\theta)-Z)\\
&=\phi(0)\,\exp{(-\vwmo(\theta-l)^2/2)}\,\exp{(-Z^2/2+\vwmh(l-\theta)Z)}~.
\end{align*}
Thus, we have,
\begin{align*}
&\ex\big[\log\big\{1+c(\eta)\exp(\vwmo\theta^2/2)\Phi(\vwmh(l-\theta)-Z)\}\cdot I\{Z \in A^c\}\big]\\
&\le\log(2)+[\log(c(\eta))]_{+}+\vwmo(\theta l - l^2/2)_{+}+\ex(Z^2)/2 +\vwmh|l-\theta|\,\ex|Z|\\
&=k_1+k_2\,\theta
\end{align*}
where $k_1,~k_2$ are constants which depend on $l$ and $r$ (through  $\vw$) but not on $\theta$.\\
\noindent For all large $\theta$ for any fixed $l$, $P(A)=1-\Phi(\vwmh(\theta-l)-1)=\tilde{\Phi}(\vwmh(\theta-l)-1)$. Thus, we have
\begin{align*}
&\ex[\log\{1+c(\eta)e^{\vwmo \theta^2/2}\Phi(\vwmh(l-\theta)-Z)\}\cdot I\{Z\in A\}]\\
&\le (1+k_3\,\vwmo\theta^2/2)\,\tilde{\Phi}(\vwmh(\theta-l)-1) \leq k_4
\end{align*}
for any fixed $l$ for all large $\theta$ values; $k_3,k_4$and $k_5$ are constants which may depend on $l$ and $r$ but not on $\theta$. This completes the proof of the lemma. \medskip\\

\noindent \textbf{Proof of Lemma~\ref{lem-SS-2}.} First note that, by definition of $W$ 
\begin{align*}
&\ex[\log\{\Phi(\vwmh l - \vw^{1/2} W) - \Phi (-\vwmh l - \vw^{1/2} W)\}] \\
&= \ex[\log\{\Phi(\vwmh(l-\theta)-Z)-\Phi(-\vwmh(l+\theta)-Z)\}]
\end{align*}
where, $Z$ has standard normal distribution. As~ $\vw\le1$ the above is bounded below by
$\ex[\log\{\Phi(l-\theta-Z)-\Phi(-(l+\theta)-Z)\}]$.
Now,  for $|\theta|\le l$, in order to  lower bound the aforementioned expression it is enough to lower bound $\ex[\log\{\Phi(-Z)-\Phi(-l-Z)\}]$ which equals 
$$\ex[\log\{\Phi(Z)-\Phi(-l+Z)\}]
\ge \ex [\log\{\Phi(Z)-\Phi(-1+Z)\}] \text{ for all } l \ge 1~.$$
The above RHS is lower bounded by
\begin{align*}
\ex [\log\{\text{min}(\phi(Z)),\phi(-1+Z))\}]
&\ge\ex [\log(\phi(Z) \phi(-1+Z))]\\
&=2\log\phi(0)-{3}/{2}~.
\end{align*}
This completes the proof.\medskip\\
\noindent \textbf{Proof of Lemma~\ref{lem-SS-3}.}
For the proof of part (a) of the lemma, note that by definition \eqref{eq:SS-decomp-1b}
%$\ex\{\log \DS_{\theta}(Z) \} \leq \log(2) + \log c(\eta) + \ex (\theta+Z)^2 $
$$\log \DS_{\theta}(Z) \leq  \log 2 + [\log c(\eta) + X^2/2]_+ \text{ where } X \sim N(\theta, 1)~,$$
where,
$\log c(\eta)=- \log \{2 \phi(0)(1-\eta)\} -\log l - \vw^{-1} \lambda^2/2~.$
Thus, we have the following bound
$$\ex\{\log \DS_{\theta}(Z)\} \leq  2^{-1}\ex [(\theta+Z)^2-\vw^{-1} \lambda^2]_+ + O(1)~,$$
where $Z$ has standard normal distribution. 
Now if  $|\theta| > \tilde{\lambda}$, then
\begin{align*}
\ex [(\theta+Z)^2-\vw^{-1} \lambda^2]_+ &\leq \ex (\theta+Z)^2-\vw^{-1} \lambda^2 \cdot P(|\theta+Z|\geq \vw^{-1/2} \lambda)\\
& \leq (\theta^2+1)-\vw^{-1} \lambda^2 \cdot P(|Z|\leq (2 \log \lambda)^{1/2})\\
& \leq \theta^2 -\vw^{-1} \lambda^2 + O(\lambda) \text{ as } \lambda \to \infty~.
\end{align*}
The above asymptotic inequality follows by using Mills ratio bounds \citep{Johnstone-book} which suggests $$P(|Z|\geq (2 \log \lambda)^{1/2}) \leq 2\,(2 \log \lambda)^{-1/2}\, \phi((2 \log \lambda)^{1/2})\leq O(\lambda^{-1}) \text{ as }\lambda \to \infty.$$ 
From above we have the desired result after noting that $\log c(\eta) \geq -[\log l]_+ - \vw^{-1}\lambda^2$.\medskip\\
Now, if  $|\theta| \leq \tilde{\lambda}$ then, 
\begin{align*}
\ex [(\theta+Z)^2-\vw^{-1} \lambda^2]_+ &\leq [\theta^2-\vw^{-1} \lambda^2]_+ + 2 |\theta| \, \ex|Z| + \ex [Z^2] \\
& \leq [\tilde{\lambda}^2-\vw^{-1}\lambda^2]_+ + 2  \, \tilde{\lambda} \, \phi(0) + 1
\end{align*}
which provides us with the stated result.\medskip\\


